Path Planning for Manipulation using Experience-driven Random Trees

Robotic systems may frequently come across similar manipulation planning problems that result in similar motion plans. Instead of planning each problem from scratch, it is preferable to leverage previously computed motion plans, i.e., experiences, to ease the planning. Different approaches have been proposed to exploit prior information on novel task instances. These methods, however, rely on a vast repertoire of experiences and fail when none relates closely to the current problem. Thus, an open challenge is the ability to generalise prior experiences to task instances that do not necessarily resemble the prior. This work tackles the above challenge with the proposition that experiences are "decomposable" and "malleable", i.e., parts of an experience are suitable to relevantly explore the connectivity of the robot-task space even in non-experienced regions. Two new planners result from this insight: experience-driven random trees (ERT) and its bi-directional version ERTConnect. These planners adopt a tree sampling-based strategy that incrementally extracts and modulates parts of a single path experience to compose a valid motion plan. We demonstrate our method on task instances that significantly differ from the prior experiences, and compare with related state-of-the-art experience-based planners. While their repairing strategies fail to generalise priors of tens of experiences, our planner, with a single experience, significantly outperforms them in both success rate and planning time. Our planners are implemented and freely available in the Open Motion Planning Library.

==> Sections/planner.tex <==
\section{EXPERIENCE-DRIVEN RANDOM TREES} \label{sec:planner}

    \begin{figure*}[ht]
        \centering
        \subfloat[ERT: first iteration example]{\includegraphics[width=0.275\textwidth, trim=0.1cm 0.0cm 0.3cm 0.3cm, clip]{./Figures/ert_1.pdf}}
        \quad
        \subfloat[ERT: \textit{explore} example]{\includegraphics[width=0.275\textwidth, trim=0.1cm 0.0cm 0.3cm 0.3cm, clip]{./Figures/ert_2.pdf}}
        \quad
        \subfloat[ERT: \textit{connect} example]{\includegraphics[width=0.275\textwidth, trim=0.1cm 0.0cm 0.3cm 0.3cm, clip]{./Figures/ert_3.pdf}} \quad
        % \subfloat[ERTConnect projected in the workspace]{\includegraphics[width=0.15\textwidth]{./Figures/Picture1.png}}
        \\
        % \subfloat[ERTConnect: first iteration]{\includegraphics[width=0.25\textwidth]{./Figures/temporal.pdf}}
        % \subfloat[ERTConnect: explore ]{\includegraphics[width=0.25\textwidth]{./Figures/temporal.pdf}}
        % \subfloat[ERTConnect: connect]{\includegraphics[width=0.25\textwidth]{./Figures/temporal.pdf}}
        % \subfloat[ERTConnect: connect]{\includegraphics[width=0.25\textwidth]{./Figures/temporal.pdf}}
        \caption{Experience-driven random trees iteratively build a tree (green) of micro-experiences. At each iteration, an existing node in the tree is randomly selected to either \textit{explore} the most suitable continuation of the task (e.g., snapshots in (a) and (b)), or \textit{connect} to another known state (e.g., the goal state as in (c) (ERT), or a state in the other tree (ERTConnect)). In both cases, relevant micro-experiences (dotted red) are generated by morphing segments (red) of the prior path experience~$\demo^\prime$.}

        %, i.e., segments that resemble those in $\demo^\prime$ ($\demo$ mapped onto the current planning problem via the \textit{connect} method).  to relevantly \textit{connect} and \textit{explore} regions of interest in $\sspace$. (a-b)~An existing node in the tree is randomly selected to \textit{explore} the most suitable continuation of the task. (c)~Given two known states, a relevant micro-experience is morphed to \textit{connect}. \textcolor{green}{change reference part in the paper}}
        %  \textcolor{red}{Generation of micro-experiences (dotted red) from segments (red) of the experience $\demo^\prime$ to relevantly \textit{connect} and \textit{explore} regions of interest in $\sspace$. $\demo^\prime$ results from mapping $\demo$ onto the current planning problem via the \textit{connect} method. These two operations constitute the core of the proposed tree sampling-based planners: the \ac{ERT} and the ERTConnect.}}
        \label{fig:illustration_connect_explore}
        \vspace{-0.35cm}
    \end{figure*}

    % The presented experience-based planner is designed specifically to leverage from a single prior experience in form of a path, i.e., ${\mathcal{L}: \demo \rightarrow \traj}$. As introduced earlier, the proposed method builds on the idea that different task instantiations require similar motion plans, which can be obtained from each other by means of a sequence of local modifications. Thus, formally, our planner seeks a path ${\traj \in [0,1] \rightarrow \sspace_\free}$ that connects a start configuration ${\traj(0) = \q_\start}$ and ${\traj(1) = \q_\goal}$ via the process ${\mathcal{L}: \decomposition \times \{{\nu}_1, ..., {\nu}_k\} \times \composition}$ subject to \eqref{eq:a_cons} and \eqref{eq:q_cons}. Our planner incrementally exploits the prior until a suitable decomposition and sequence of modulations that compose a solution, i.e., ${\traj = \bigcup_{i=1}^k \nu_i({\demosegment}_i)}$, is found. The underlying process through which we exploit the prior experience to generate task-relevant segments (micro-experiences) is detailed in \sref{sec:planner_segment}. This core routine is employed in a uni- and bi-directional sampling-based planning strategy, respectively introduced in \sref{sec:planner_uni} and \sref{sec:planner_bi}.


    The presented experience-driven random tree planners (ERT and ERTConnect) are inspired by tree sampling-based methods~\cite{hsu1997path,kuffner2000rrt}. Our planners, however, leverage a single task-relevant prior path experience to
    %guide the search of the \mbox{$\cspace$-space} connectivity in a task-relevant manner.
    % capture the connectivity of the space in a task-relevant manner.
    ease the capture of connectivity of the space.
    % This experience-driven search derives from the (de)composability and malleability procedures formalised in \sref{sec:gme}.
    % Such experience-driven connectivity derives from incrementally exploiting a given prior $\demo$ to build a tree whose edges are segments (micro-experiences) that resemble those in $\demo^\prime$ ($\demo$ mapped onto the current planning problem, see \fref{fig:illustration_connect_explore}).
    % Such experience-driven connectivity search is conducted by incrementally exploiting a given prior $\demo$ to build a tree of micro-experiences (see green tree in \fref{fig:illustration_connect_explore}).
    Such prior path experience $\demo$ is exploited incrementally to build a tree of micro-experiences (see green tree in \fref{fig:illustration_connect_explore}). The micro-experiences in the tree resemble those in $\demo^\prime$ ($\demo$ mapped onto the current planning problem), such that a trace along the tree edges corresponds to a sequence of local modifications ${\decomposition \times \{{\nu}_1, ..., {\nu}_k\} \times \composition}$ on $\demo^\prime$ subject to \eqref{eq:a_cons}, \eqref{eq:segment_transform}, and \eqref{eq:q_cons}. Therefore, formally, the planner seeks a suitable experience decomposition and sequence of modulations that compose a solution, i.e., ${\traj = \bigcup_{i=1}^k \nu_i({\demosegment}_i)}$, that satisfies ${\traj \in [0,1] \rightarrow \sspace_\free}$, ${\traj(0) = \q_\start}$ and ${\traj(1) = \q_\goal}$.

    The core routine through which the planner exploits the prior experience to generate task-relevant micro-experiences is detailed in \sref{sec:planner_segment}, and its usage in a uni- and bi-directional sampling-based planning strategy is presented in \sref{sec:planner_uni} and \sref{sec:planner_bi}, respectively. Finally, we discuss the parametrisation of both planners in \sref{sec:planner_parameters}.

    % \textcolor{red}{discuss why not RRTconnect}

    % \begin{figure}[b!]
    %     \centering
    %     \subfloat[\textit{connect:} infer a suitable connection for the states $\s_\init$ and $\s_\targ$]{\includegraphics[width=0.9\columnwidth]{./Figures/connect.pdf}} \\
    %     \subfloat[\textit{explore:} infer a suitable continuation of the robot-task state $\s_\init$]{\includegraphics[width=0.9\columnwidth]{./Figures/explore.pdf}}
    %     % \caption{Illustration about the generation of micro-experiences to relevantly \textit{connect} and \textit{explore} different regions of interest in $\sspace$. These two operations constitute the core of the proposed experience-based \ac{ERT} and ERTConnect planners.}
    %     \caption{Generation of micro-experiences (dotted red) from segments (red) of the experience $\demo^\prime$ to relevantly \textit{connect} and \textit{explore} regions of interest in $\sspace$. $\demo^\prime$ results from mapping $\demo$ onto the current planning problem via the \textit{connect} method. These two operations constitute the core of the proposed tree sampling-based planners: the \ac{ERT} and the ERTConnect.}
    %     \label{fig:illustration_connect_explore}
    % \end{figure}

    % We formulate a joint extraction and mapping of micro-experiences to

    % jointly extracts relevant segments and suitable mappings

    % to explore a suitable ${\traj = \bigcup_{i=1}^k \nu_i({\demosegment}_i)}$


    %As formulated in \sref{sec:problem_formulation}, we approach this challenge by formulating a three-fold procedure that (i)~decomposes the prior experience into a random set of segments, (ii)~applies a random-bounded transformation to them, and finally (iii)~composes the resulting segments. These three steps are jointly addressed in the proposed planner.

    %Formally, as introduced in \sref{sec:problem_formulation}, we approach this challenge by formulating a three-fold procedure that (i)~decomposes the prior experience into a random set of segments, (ii)~applies a random-bounded transformation to them, and finally (iii)~composes the resulting segments. These three steps are jointly addressed in the proposed planner. %This section introduces the uni- and bi-directional versions of the proposed method.

    % ===============================
    % ===============================
    % ===============================
    % \subsection{Overview \label{sec:preliminaries_pf}}
    %     %The motion planning problem considered in this manuscript seeks a continuous collision-free path ${\xi \in [0,1]}$ connecting a start configuration $\q_{start}$ to a goal configuration $\q_{goal}$, such that ${\xi(0) = \q_{start}}$ and ${\xi(1) = \q_{goal}}$.

    %     \textcolor{red}{piecewise-continuous path}

    %     Therefore, the motion planning problem formulated in this manuscript is to find a suitable process ${\mathcal{L}: \mathrm{C}^{-1} \times \{{\nu}_1, ..., {\nu}_k\} \times \mathrm{C}}$, $k$ being undefined and $\mathcal{L}$ subject to \eqref{eq:q_cons}, \eqref{eq:a_cons} and \eqref{eq:e_cons}, such that a robot can leverage from a prior experience $\demo$ to solve task-related planning problems. Formally, this involves to jointly explore a suitable decomposition $\mathrm{C}^{-1}$ of $\demo$ and the corresponding local process $\nu$ such that, the composition $\mathrm{C}$ of the obtained segments $\psi^\prime$:
    %     \begin{align}
    %         \traj = &\bigcup_{i=1}^k \nu_i(\psi_i), \label{eq:pf}
    %     \end{align}
    %     results in a valid solution $\traj$ of the current task instance. $\traj$ is a valid solution of the planning problem if it is a continuous collision-free path ${\traj \in [0,1] \rightarrow \cspace_\text\free}$ that connects a start configuration ${\traj(0) = \q_\start}$ and ${\traj(1) = \q_\goal}$.

    %     \textcolor{red}{we propose this strategy in uni- and bi-directional fashion}

        %As there possibly exist multiple paths $\traj$ satisfying the requirements of the planning problem, the threefold modulation $H$ is not unique but a one-to-many mapping.

    % ===============================
    % ===============================
    % ===============================
    % \subsection{Task-relevant Micro-\textcolor{red}{motions} via Local Modulators \label{sec:planner_segment}}
    \subsection{Generating Task-relevant Micro-experiences \label{sec:planner_segment}}% -- Joint Segment and Transform Sampling \label{sec:planner_segment}}
    %\subsection{Affine Transformations as Local Modulators -- Joint Segment and Transform Sampling \label{sec:planner_segment}}

        %For planning purposes, we are particularly interested in generating task-relevant micro-experiences that allow to \textit{connect} and \textit{explore} task-relevant parts of $\sspace$. The former seeks \textit{which is the best way to connect two particular states?}, and the latter \textit{which is the best way to continue from this state?}.

        % \aref{alg:segment} encompasses both operations. If a $\s_\targ$ is provided (\lref{alg_line:gs_conditional}), a relevant micro-experience is generated to \textit{connect} $\s_\init$ with $\s_\targ$ (\lalref{alg_line:gs_connect_extract}{alg_line:gs_connect_tss}). Otherwise, a micro-experience is generated to relevantly \textit{explore} $\sspace$ from $\s_\init$ (\lalref{alg_line:gs_explore_sample_end}{alg_line:gs_explore_tss}). Each process extracts a suitable segment from $\demo$ and estimates the parameters $\tss$ and $\tsb$ for employing \eref{eq:segment_transform}, such that the mapping of the segment results onto the region of interest (\lref{alg_line:gs_map}). \fref{fig:illustration_connect_explore} illustrates both operations.

        For planning purposes, we are particularly interested in generating micro-experiences that are task-relevant in $\sspace$, i.e., coherent according to the robot state in a task. \aref{alg:segment} leverages the prior path $\demo^\prime$ to infer micro-experiences that are suitable to either \textit{connect} two particular states $\s_\init$ and $\s_\targ$ (\ltlref{alg_line:gs_connect_unpack}{alg_line:gs_connect_tss}), or \textit{explore} the best way to continue the task from a given state $\s_\init$ (\ltlref{alg_line:gs_explore_sample_end}{alg_line:gs_explore_tss}). These two processes, which are illustrated in \fref{fig:illustration_connect_explore},
        %and detailed next,
        employ the path decomposability and malleability introduced in \sref{sec:preliminaries_de_composability} and \sref{sec:preliminaries_malleability}, respectively, to extract and map segments of $\demo^\prime$ onto any region of interest in $\sspace$ (\lref{alg_line:gs_map}) via the affine morphing in~\eref{eq:segment_transform} referred to as \method{TRANSFORM\_SEGMENT}{$\cdot$}.

         \begin{algorithm}[b!]
            \SetInd{0.5em}{0.5em}
            \DontPrintSemicolon

            %this is the mapping algorithm that does tree -> demonstration -> tree, i.e. the unique part of the algorithm that uses the demonstration

            \caption{\mbox{GENERATE\_SEGMENT($\s_\init$, $\s_\targ$, $\demo^\prime$)}}
            \label{alg:segment}

            \nonl\textbf{Input:} \\
            \nonl\forceindent$\s_\init$: required segment configuration-phase start \\
            \nonl\forceindent$\s_\targ$: required segment configuration-phase end \\
            \nonl\forceindent$\demo^\prime$: prior experience \\

            \nonl\textbf{Output:} \\
            \nonl\forceindent$\psi$: generated segment \\
            \nonl\forceindent$\psi(\alpha_\targ)$: segment end configuration-phase \\

            \algspacing

            $\langle \q_\init, \alpha_\init \rangle = \s_\init$ \\

            \If(\tcp*[f]{connect}){\KwNot $\s_\targ = \varnothing$ \label{alg_line:gs_conditional}} {
                $\langle \q_\targ, \alpha_\targ \rangle = \s_\targ$ \label{alg_line:gs_connect_unpack} \\
                $\demosegment \leftarrow \demo^\prime(\alpha_\init$, $\alpha_\targ)$ \label{alg_line:gs_connect_extract} \\
                % $\tsb \leftarrow \dist(\q_\init$, $\demosegment(\alpha_\init))$ \label{alg_line:gs_connect_tsb} \\
                % $\tss \leftarrow \dist(\q_\targ$, $\q_\init \cup \demosegment)$ \label{alg_line:gs_connect_tss}
                $\tsb \leftarrow \q_\init - \demosegment(\alpha_\init)$ \label{alg_line:gs_connect_tsb} \\
                $\tss \leftarrow \q_\targ - (\demosegment(\alpha_\targ) + \tsb)$ \label{alg_line:gs_connect_tss}
            }
            \Else(\tcp*[f]{explore}) {
                $\alpha_\targ \leftarrow$ \method{SAMPLE\_SEGMENT\_END}{$\alpha_\init$} \label{alg_line:gs_explore_sample_end} \\

                % \textcolor{red}{sample end segment is different depending on the tree!} \\
                % $\alpha_\targ = \min\left(\alpha_\init + \mathbb{U}\left(\alpha_\alphamin, \; \alpha_\alphamax\right), \; 1\right)$ \\
                % $\alpha_\targ = \max\left(0, \; \alpha_\init - \mathbb{U}\left(\alpha_\alphamin, \; \alpha_\alphamax\right)\right)$ \\
                % \textcolor{red}{sample end segment is different depending on the tree!} \label{alg_line:gs_explore_sample_end} \\

                $\demosegment \leftarrow \demo^\prime(\alpha_\init, \; \alpha_\targ)$ \label{alg_line:gs_explore_extract} \\
                % $\tsb \leftarrow \dist(\q_\init, \; \demosegment(\alpha_\init))$ \label{alg_line:gs_explore_tsb} \\
                $\tsb \leftarrow \q_\init - \demosegment(\alpha_\init)$ \label{alg_line:gs_explore_tsb} \\
                $\tss \leftarrow \mathbb{U}(-\tse |{\demosegment}_\alpha|, \; \tse |{\demosegment}_\alpha|)$ \label{alg_line:gs_explore_tss}
            }
            $\psi \leftarrow$ \method{TRANSFORM\_SEGMENT}{$\demosegment$, $\tss$, $\tsb$} \label{alg_line:gs_map} \tcp*[f]{\eref{eq:segment_transform}} \\
            % \KwReturn $\psi^\prime$, $\s_\targ$
            \KwReturn $\langle\psi, \; \psi(\alpha_\targ)\rangle$
        \end{algorithm}

        % ===============================
        % ===============================
        % \textcolor{green}{Case 1: given target, RESTRICTIVE tree expansion (Algorithm 2, line 3 and 4)}  \\
        \textit{Connect} (\ltlref{alg_line:gs_connect_unpack}{alg_line:gs_connect_tss}): given two task-related configuration-phase states ${\s_\init = \langle \q_\init, \alpha_\init \rangle}$ and ${\s_\targ = \langle \q_\targ, \alpha_\targ \rangle}$, we hypothesise that a suitable connection
        % of these states
        may result from mapping the micro-experience ${\demosegment: \alpha \in [\alpha_\init, \alpha_\targ]}$ between $\s_\init$ and $\s_\targ$.
        Thus, after extracting the relevant micro-experience from
        % the mapped prior experience
        $\demo^\prime$
        % as introduced in \sref{sec:preliminaries_de_composability}
        (\lref{alg_line:gs_connect_extract}), the parameters $\tsb$ and $\tss$ of the mapping in \eref{eq:segment_transform} are calculated such that the resulting micro-experience~$\psi$ satisfies ${\psi(\alpha_\init) = \q_\init}$ and ${\psi(\alpha_\targ) = \q_\targ}$ (\lalref{alg_line:gs_connect_tsb}{alg_line:gs_connect_tss}).


        % ===============================
        % ===============================
        %\textcolor{green}{Case 2 : NOT given target, FREE tree expansion (Algorithm 2, line 6 to 8)} \\

        %  given a configuration $\q_\init$ with task phase $\alpha_\init$, we seek a segment $\psi^\prime$ that explores (continues) the task reasonably (i.e. not exactly replicating the demonstration, nor being completely different).

        \textit{Explore} (\ltlref{alg_line:gs_explore_sample_end}{alg_line:gs_explore_tss}): given one task-related configuration-phase state ${\s_\init = \langle \q_\init, \alpha_\init \rangle}$, we hypothesise that a suitable continuation of the task is to apply a micro-experience similar to that ${\demosegment \in \demo^\prime}$ starting at $\alpha_\init$. For that, we first determine which span of $\demo^\prime$ to exploit by defining $\alpha_\targ$ (\lref{alg_line:gs_explore_sample_end}). An appropriate $\alpha_\targ$ depends on the direction in which $\demo^\prime$ is being exploited; we call it \texttt{forward} when exploiting the prior from $\demo^\prime(0)$ to $\demo^\prime(1)$, and \texttt{backward} otherwise. Correspondingly, \method{SAMPLE\_SEGMENT\_END}{$\alpha_\init$} defines $\alpha_\targ$ as:
        \begin{align} \raisetag{4.6ex}
            \!\!\!\!
            \resizebox{0.93\columnwidth}{!}{$%
            \alpha_\targ =
            \begin{cases}
                \min\left(\alpha_\init + \mathbb{U}\left(\psl, \; \psu\right), \; 1\right), & \text{if} \; \texttt{forward} \\
                \max\left(0, \; \alpha_\init - \mathbb{U}\left(\psl, \; \psu\right)\right), & \text{if} \; \texttt{backward}
            \end{cases}
            $}
        \end{align}
        % where $\mathbb{U}(\psl, \psu)$ draws a sample from a uniform distribution between some user-defined lower and upper bound $\psl$ and $\psu$. These bounds delimit the level of granularity and randomness for the exploitation of the experience $\demo^\prime$.
        where $\mathbb{U}(\psl, \psu)$ draws a sample from a uniform distribution to determine the phase span of the extracted segment. The bounds $\psl$ and $\psu$ are discussed in \sref{sec:planner_parameters}.


        Next, the corresponding segment ${\demosegment: \alpha \in [\alpha_\init, \alpha_\targ]}$ is extracted from the mapped prior path experience $\demo^\prime$ (\lref{alg_line:gs_explore_extract}). As such micro-experience is to be leveraged from $\s_\init$, $\tsb$ is computed for the resulting micro-experience $\psi$ to satisfy ${\psi(\alpha_\init) = \q_\init}$ (\lref{alg_line:gs_explore_tsb}). Then, the shearing coefficient $\tss$ is sampled randomly within some bounds to generate a micro-experience similar to $\demosegment$ (\lref{alg_line:gs_explore_tss}). In particular, $\tss$ is drawn from a uniform distribution $\mathbb{U}\left(-\tse |{\demosegment}_\alpha|, \; \tse |{\demosegment}_\alpha|\right)$ such that: %with user-defined boundary $\pm\tse|\psi|$, such that
        \begin{align}
            \psi(\alpha) - (\demosegment(\alpha) + \tsb) \leq \tse |{\demosegment}_\alpha| \quad \forall \; \alpha \in [\alpha_\init, \alpha_\fin],
            \label{eq:e_cons}
        \end{align}
        where $\tse$ is a user-defined malleability bound that, intuitively, defines the volume (neighbourhood) around the provided $\demosegment$ that the planner can explore (see \sref{sec:planner_parameters}). Such upper bound in \eqref{eq:e_cons} is scaled by the segment's phase span such that the accumulated deformation along the resulting path does not exceed $\tse$.

        Overall, the method \method{GENERATE\_SEGMENT}{$\cdot$} enables the presented experience-guided random tree planners to leverage a single path experience at different levels of granularity, and map task-relevant segments onto any region of interest in~$\sspace$. The remaining of this section discusses the usage of such routine in a uni-directional (ERT) and a bi-directional (ERTConnect) tree sampling-based technique.

    % ===============================
    % ===============================
    % ===============================
    \subsection{Uni-directional Experience-driven Random Trees (ERT) \label{sec:planner_uni}}

        \begin{algorithm}[t!]
            \SetInd{0.5em}{0.5em}
            \DontPrintSemicolon
            \caption{ERT($\s_\start$, $\s_\goal$, $\demo$)} \label{alg:evs}

            \nonl\textbf{Input:} \\
            % \nonl\forceindent$\s_\start$: start configuration-phase \\
            % \nonl\forceindent$\s_\goal$: goal configuration-phase \\
            \nonl\forceindent$\s_\start$ and $\s_\goal$: start and goal configuration-phase \\
            \nonl\forceindent$\demo$: prior experience \\

            \nonl\textbf{Output:} \\
            \nonl\forceindent$\xi$: collision-free path \\

            \algspacing
            \tcc{map $\demo$ onto current problem}
            $\langle\demo^\prime, \, \varnothing\rangle \leftarrow$ \method{GENERATE\_SEGMENT}{$\s_\start$, $\s_\goal$, $\demo$} \label{alg_line:evs_pro1} \\
            \If{\method{IS\_VALID}{$\demo^\prime$} \label{alg_line:evs_pro2}} {
                \KwReturn $\demo^\prime$
            }

            \algspacing
            \tcc{sampling-based $\demo^\prime$ exploitation}
            $\tree$.init($\s_\start$) \;
            \While{\KwNot \method{STOPPING\_CONDITION}{} \label{alg_line:evs_sc}} {
                \tcc{node selection}
                $\s_\init \leftarrow$ $\tree$.\method{select\_node}{} \label{alg_line:evs_ns}

                \algspacing
                \tcc{micro-experience generation}
                $\s_\targ \leftarrow \varnothing$ \label{alg_line:evs_ss_start} \\
                \If{\method{ATTEMPT\_GOAL}{} = True} {
                    $\s_\targ \leftarrow \s_\goal$
                }
                $\langle\psi, \, \s_\targ\rangle \leftarrow$ \method{GENERATE\_SEGMENT}{$\s_\init$, $\s_\targ$, $\demo^\prime$} \label{alg_line:evs_ss_end}

                \algspacing
                \tcc{tree extension}
                \If{\method{EXTEND}{$\tree$, $\psi$, $\s_\init$, $\s_\targ$}  $\neq$ Trapped \label{alg_line:evs_te_extend}} {
                    \If{\method{GOAL\_REACHED}{$\s_\targ$} \label{alg_line:evs_te_goal}} {
                        \KwReturn \method{PATH}{$\tree$} \label{alg_line:evs_te_return}
                    }
                }
            }
        \end{algorithm}




        \aref{alg:evs} provides the pseudo-code of the uni-directional version of our planner. The algorithm seeks finding a continuous path from a start $\s_\start$ to a goal $\s_\goal$ configuration, given a related path experience $\demo$. The planner firstly maps the entire prior experience ${\nu: \demo \rightarrow \demo^\prime}$ onto the current planning problem
        %defined by $\s_\init$ and $\s_\goal$
        (\lref{alg_line:evs_pro1}).
        If $\demo^\prime$ is not valid (\lref{alg_line:evs_pro2}), the planner proceeds to exploit $\demo^\prime$ to generate task-relevant micro-experiences. The planner follows a three-step procedure (node selection, segment sampling, and tree extension) until the stopping condition is met (\lref{alg_line:evs_sc}). A node $\s_\init$ is selected from the tree $\tree$ with probability ${P(node) = \frac{1}{w(node)+1}}$ (\lref{alg_line:evs_ns}), where $w(\cdot)$ is a weighting function that penalises the selection of a node according to the number of times that it has already been selected. This weighted sampling strategy promotes a uniform selection of all nodes over time, thus promoting a first depth exploration of the task phase~$\alpha$.
        % From the selected node $\s_\init$, the tree is expanded following the path (de)composability intuition given earlier in this manuscript. This is, the tree is expanded using segments that are similar to those in the prior experience $\demo$.
        From the selected node $\s_\init$, the tree is expanded using segments that resemble those in the prior experience~$\demo^\prime$.
        With probability $\tsg$, the expansion of the tree attempts to connect $\s_\init$ with $\s_\goal$, whereas with probability $(1-\tsg)$ the expansion is done towards a semi-random configuration $\s_\targ$ (\ltlref{alg_line:evs_ss_start}{alg_line:evs_ss_end}). \aref{alg:segment}, previously explained in \sref{sec:planner_segment}, details the extraction of suitable segments under these two different cases. The extracted segment is used to attempt expanding the tree (\lref{alg_line:evs_te_extend}) following \aref{alg:extend}. If the segment is valid,
        %(\lref{alg_line:extend_valid}),
        it is integrated into the tree.
        %(\lalref{alg_line:extend_integrate_start}{alg_line:extend_integrate_end}).
        Note that the connection between states is a micro-experience whose shape is similar to the related one in the prior experience, not a straight line. Finally, if the incorporated (valid) segment reaches the goal, the path is returned (\lalref{alg_line:evs_te_goal}{alg_line:evs_te_return}).



        \begin{algorithm}[t!]
            \SetInd{0.5em}{0.5em}
            \DontPrintSemicolon

            \caption{EXTEND($\tree$, $\psi$, $\s_\init$, $\s_\targ$)}
            \label{alg:extend}

            \nonl\textbf{Input:} \\
            \nonl\forceindent$\tree$: tree of previously generated micro-experiences \\
            \nonl\forceindent$\psi$: new generated micro-experience \\
            % \nonl\forceindent$\s_\init$: start configuration-phase of segment $\psi$ \\
            % \nonl\forceindent$\s_\targ$: end configuration-phase of segment $\psi$ \\
            \nonl\forceindent$\s_\init$ and $\s_\targ$: start and end configuration-phase of $\psi$ \\

            \nonl\textbf{Output:} \\
            \nonl\forceindent outcome of the tree extension attempt \\

            % $\psi' \leftarrow$ \method{TRANSFORM\_SEGMENT}{$\psi$, $\q_\init$, $\q_\targ$}

            \algspacing
            \If{\method{IS\_VALID}{$\psi$} \label{alg_line:extend_valid}} {
                $\tree$.\method{add\_vertex}{$\s_\targ$} \label{alg_line:extend_integrate_start} \;
                $\tree$.\method{add\_edge}{$\psi$, $\s_\init$, $\s_\targ$} \label{alg_line:extend_integrate_end} \;
                \KwReturn Advanced
            }
            \KwReturn Trapped
        \end{algorithm}









    % ===============================
    % ===============================
    % ===============================
    \subsection{Bi-directional ERT (ERTConnect) \label{sec:planner_bi}}

        \begin{algorithm}[t!]
            \SetInd{0.5em}{0.5em}
            \DontPrintSemicolon
            \caption{ERTConnect($\s_\start$, $\s_\goal$, $\demo$)} \label{alg:evsconnect}

            \nonl\textbf{Input:} \\
            % \nonl\forceindent$\s_\start$: start configuration-phase \\
            % \nonl\forceindent$\s_\goal$: goal configuration-phase \\
            \nonl\forceindent$\s_\start$ and $\s_\goal$: start and goal configuration-phase \\
            \nonl\forceindent$\demo$: prior experience \\

            \nonl\textbf{Output:} \\
            \nonl\forceindent$\xi$: collision-free path \\

            \algspacing
            \tcc{map $\demo$ onto current problem}
            $\langle\demo^\prime, \; \varnothing\rangle \leftarrow$ \method{GENERATE\_SEGMENT}{$\s_\start$, $\s_\goal$, $\demo$} \label{alg_line:evs_connect_pro1} \\
            \If{\method{IS\_VALID}{$\demo^\prime$} \label{alg_line:evs_connect_pro2}} {
                \KwReturn $\demo^\prime$
            }

            \algspacing

            \tcc{sampling-based $\demo^\prime$ exploitation}
            $\tree_a$.init($\s_\start$) \label{alg_line:evs_connect_setup1} \;
            $\tree_b$.init($\s_\goal$) \label{alg_line:evs_connect_setup2} \;
            \While{\KwNot \method{STOPPING\_CONDITION}{} \label{alg_line:evsconnect_sc}} {
                \tcc{node selection}
                $\s_\init \leftarrow$ $\tree_a$.\method{select\_node}{} \label{alg_line:evsconnect_ns} %\tcc{weighted selection}

                \algspacing
                \tcc{micro-experience generation}
                $\langle\psi, \; \s_\targ\rangle \leftarrow$ \method{GENERATE\_SEGMENT}{$\s_\init$, $\varnothing$, $\demo^\prime$} \label{alg_line:evsconnect_ss}

                \algspacing

                \tcc{tree extension}
                \If{\method{EXTEND}{$\tree_a$, $\psi$, $\s_\init$, $\s_\targ$} $\neq$ Trapped \label{alg_line:evsconnect_extend1}} {
                    \If{\method{OTHER\_EXTREME\_REACHED}{$\s_\targ$} \label{alg_line:evsconnect_return1_start}} {
                        \KwReturn \method{PATH}{$\tree_a$} \label{alg_line:evsconnect_return1_end}
                    }

                    \algspacing
                    \tcc{micro-experience generation}
                    % $\s_\targ \leftarrow$ $\tree_b$.\method{nearest\_neighbour}{$\s_\targ$} \label{alg_line:evsconnect_nearest}

                    $\s_\near \leftarrow$ $\tree_b$.\method{nearest\_neighbour}{$\s_\targ$} \label{alg_line:evsconnect_nearest}

                    % $\psi \leftarrow$ \method{EXTRACT\_SEGMENT}{$\demo$, $\q_\init$, $\q_\targ$}

                    % \mbox{$\langle\psi, \; \s_\targ\rangle \leftarrow$ \method{GENERATE\_SEGMENT}{$\s_\targ, $\s_\targ$, $\demo^\prime$} \label{alg_line:evsconnect_ct}}

                    \mbox{$\langle\psi, \; \s_\targ\rangle \leftarrow$ \method{GENERATE\_SEGMENT}{$\s_\near$, $\s_\targ$, $\demo^\prime$} \label{alg_line:evsconnect_ct}}

                    \algspacing

                    \tcc{tree connection}
                    % \If{\method{EXTEND}{$\tree_b$, $\psi$, $\s_\targ$, $\s_\targ$} $\neq$ Trapped \label{alg_line:evsconnect_extend2}} {
                    %     \KwReturn \method{PATH}{$\tree_a$, $\tree_b$} \label{alg_line:evsconnect_return2}
                    % }

                    \If{\method{EXTEND}{$\tree_b$, $\psi$, $\s_\near$, $\s_\targ$} $\neq$ Trapped \label{alg_line:evsconnect_extend2}} {
                        \KwReturn \method{PATH}{$\tree_a$, $\tree_b$} \label{alg_line:evsconnect_return2}
                    }
                    %}
                }
                \method{SWAP}{$\tree_a$, $\tree_b$}
            }
        \end{algorithm}

        The principles of leveraging from a prior experience by generation of task-relevant micro-experiences can also be employed in a bi-directional fashion. The proposed bi-directional planning scheme resembles, in spirit, that of the RRTConnect~\cite{kuffner2000rrt}, but with the peculiarities of our experience-based planning approach. As shown in \aref{alg:evsconnect}, the planner firstly maps the prior path experience ${\nu: \demo \rightarrow \demo^\prime}$ onto the current planning problem (\lref{alg_line:evs_connect_pro1}). If $\demo^\prime$ is not valid (\lref{alg_line:evs_connect_pro2}), the planner proceeds to exploit $\demo^\prime$ to compute a solution. The planner simultaneously grows two trees, one rooted at $\s_\start$ and the other at $\s_\goal$ (\lalref{alg_line:evs_connect_setup1}{alg_line:evs_connect_setup2}). At each iteration, until the stopping criterion is met (\lref{alg_line:evsconnect_sc}), a node of the active tree $\tree_a$ is selected via weighted selection (\lref{alg_line:evsconnect_ns}) to explore the space via a task-relevant micro-experience (\lref{alg_line:evsconnect_ss}). If the active tree is extended successfully with the generated segment (\lref{alg_line:evsconnect_extend1}), we first check whether the end of the motion has reached the other extreme (\lref{alg_line:evsconnect_return1_start}). This implies that a path has been found before the trees connected, either by $\tree_a$ reaching the root of $\tree_b$ or the other way around, in which case the path is returned as a solution (\lref{alg_line:evsconnect_return1_end}). Otherwise, the node of $\tree_b$ nearest to $\s_\targ$ is selected
        % as target node
        (\lref{alg_line:evsconnect_nearest}) to attempt unifying both trees with a task-relevant segment (\lref{alg_line:evsconnect_ct}). If the extension is successful, the corresponding path is returned (\lalref{alg_line:evsconnect_extend2}{alg_line:evsconnect_return2}).

    % ===============================
    % ===============================
    % ===============================
    \subsection{Planner's Parameterisation \label{sec:planner_parameters}}
        Next, we review the parameters of the presented planners:
        % The presented planners have some parameters which can be used to control their behaviour as discussed next:
        \begin{itemize}
            \item $\tsg$ - probability of attempting to \textit{connect} the tree to the goal (only in ERT). This parameter should be set small to allow the planner \textit{explore} the space. Default: ${\tsg = 0.05}$.
            \item $\psl$ and $\psu$ - lower and upper phase span bounds of the extracted segments. Indirectly, these parameters delimit the length of the motions added in the tree to \textit{explore} the space. Default: ${\psl=0.05}$ and $\psu={0.1}$.
            \item $\tse$ - malleability bound to delimit the amount of morphing applied to the micro-experiences. Intuitively, this parameter defines a volume around the mapped path $\demo^\prime$ where the planner can \textit{explore} for a solution.
            Default: ${\tse = \textbf{5}_{1\times n}}$ (large enough to cover the entire robot's kinematic range).
        \end{itemize}

        % \textcolor{blue}{These bounds delimit the level of granularity and randomness for the exploitation of the experience $\demo^\prime$.}

        Our planners' default parameters are non-optimised for a particular planning problem, but left generic to succeed in many scenarios provided a relevant path experience. The planners' behaviour can be adjusted by tuning, namely, $\psl$, $\psu$ and $\tse$. As our planner discards motions that are not entirely valid, large phase spans might endanger the ability to build a tree. However, in scenarios with few obstacles, $\psl$ and $\psu$ can be set large to speed up planning computations. Also, lowering $\tse$ can speed up computations, as the tree growth would be more guided around the mapped experience~$\demo^\prime$. The lower $\tse$, the more dependant the planner is on the suitability of the provided experience. Knowing the level of dissimilarity between the experience and the current problem might aid in tuning $\tse$ to trade growth guidance and space exploration.

        % \textcolor{red}{and ours is set with some non-optimised parametrisation ${\alpha_\alphamin = 0.05}$ and ${\alpha_\alphamax = 0.1}$ to extract segments with phase span between $5\%$ and $10\%$ of the experience, and ${\tse = \textbf{5}_{1\times8}}$ to cover all the robot's kinematic range; the effect of these parameters on the planner's performance is left for future work}
    % }

        %\textcolor{red}{missing constraints on the NN, i.e. that in can only be in increasing alpha (for ta), or decreasing alpha (tb)}
        %among all nodes of $\tree_b$ that natural evolution of the task phase $\alpha$

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % NOT REALLY DONE, BUT IT MIGHT BE WORTH EXPLORING
        %   (it can lead to better quality solutions,
        %         as 'going back' is not allowed)
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % The distance metric to select nearest neighbours in the bi-directional depends on the tree that is being expanded. For the tree rooted at $\q_\start$:
        % \begin{align}
        %     \dist(\s_\targ, \s_\targ) =
        %         \begin{cases}
        %             ||\q_\targ - \q_\targ||, & \text{if} \; \alpha_\targ - \alpha_\targ \geq 0 \\
        %             \infty, & \text{otherwise}
        %         \end{cases}
        % \end{align}
        % while for the tree expanding from $\q_\goal$:
        % \begin{align}
        %     \dist(\s_\targ, \s_\targ) =
        %         \begin{cases}
        %             ||\q_\targ - \q_\targ||, & \text{if} \; \alpha_\targ - \alpha_\targ \leq 0 \\
        %             \infty, & \text{otherwise}
        %         \end{cases}
        % \end{align}

